Highly-parallelized simulation of a pixelated LArTPC on a GPU

The rapid development of general-purpose computing on graphics processing units (GPGPU) is allowing the implementation of highly-parallelized Monte Carlo simulation chains for particle physics experiments. This technique is particularly suitable for the simulation of a pixelated charge readout for time projection chambers, given the large number of channels that this technology employs. Here we present the first implementation of a full microphysical simulator of a liquid argon time projection chamber (LArTPC) equipped with light readout and pixelated charge readout, developed for the DUNE Near Detector. The software is implemented with an end-to-end set of GPU-optimized algorithms. The algorithms have been written in Python and translated into CUDA kernels using Numba, a just-in-time compiler for a subset of Python and NumPy instructions. The GPU implementation achieves a speed up of four orders of magnitude compared with the equivalent CPU version. The simulation of the current induced on $10^3$ pixels takes around 1 ms on the GPU, compared with approximately 10 s on the CPU. The results of the simulation are compared against data from a pixel-readout LArTPC prototype.

==> CUDA paper/acknowledgments.tex <==
\acknowledgments

% We would like to express our gratitude to the ArgonCube consortium and to the University of Bern for commissioning and operating the Module-0 detector.

%
% Standard piece for all FNAL-based experiments
%
This document was prepared by the DUNE collaboration using the
resources of the Fermi National Accelerator Laboratory 
(Fermilab), a U.S. Department of Energy, Office of Science, 
HEP User Facility. Fermilab is managed by Fermi Research Alliance, 
LLC (FRA), acting under Contract No. DE-AC02-07CH11359.

%
% Funding agencies, alphabetical by country, then alphabetical by agency name
%
This work was supported by
CNPq,
FAPERJ,
FAPEG and 
FAPESP,                         Brazil;
CFI, 
IPP and 
NSERC,                          Canada;
CERN;
M\v{S}MT,                       Czech Republic;
ERDF, 
H2020-EU and 
MSCA,                           European Union;
CNRS/IN2P3 and
CEA,                            France;
INFN,                           Italy;
FCT,                            Portugal;
NRF,                            South Korea;
CAM, 
Fundaci\'{o}n ``La Caixa'',
Junta de Andaluc\'ia-FEDER,
MICINN, and
Xunta de Galicia,               Spain;
SERI and 
SNSF,                           Switzerland;
T\"UB\.ITAK,                    Turkey;
The Royal Society and 
UKRI/STFC,                      United Kingdom;
DOE and 
NSF,                            United States of America.
%
% Acknowledgement of NERSC if those resources were used
%
This research used resources of the 
National Energy Research Scientific Computing Center (NERSC), 
a U.S. Department of Energy Office of Science User Facility 
operated under Contract No. DE-AC02-05CH11231.
%

We are also thankful to Max Katz from NVIDIA\textregistered~and Daniel Margala from NERSC for the precious suggestions.
%\paragraph{Note added.} This is also a good position for notes added  after the paper has been written.

==> CUDA paper/authors.tex <==
% JINST-style author list produced at 2022-11-24, from master list generated at 2022-11-22
%
\usepackage[symbol]{footmisc}

\collaboration{The DUNE Collaboration}
%----------------------------------------------------
% Institutions in alphabetical order
\affiliation[0]{Abilene Christian University, Abilene, TX 79601, USA}
\affiliation[1]{University of Albany, SUNY, Albany, NY 12222, USA}
\affiliation[2]{University of Amsterdam, NL-1098 XG Amsterdam, The Netherlands}
\affiliation[3]{Antalya Bilim University, 07190 D{\"o}{\c{s}}emealt{\i}/Antalya, Turkey}
\affiliation[4]{University of Antananarivo, Antananarivo 101, Madagascar}
\affiliation[5]{Universidad Antonio Nari{\~n}o, Bogot{\'a}, Colombia}
\affiliation[6]{Argonne National Laboratory, Argonne, IL 60439, USA}
\affiliation[7]{University of Arizona, Tucson, AZ 85721, USA}
\affiliation[8]{Universidad Nacional de Asunci{\'o}n, San Lorenzo, Paraguay}
\affiliation[9]{University of Athens, Zografou GR 157 84, Greece}
\affiliation[10]{Universidad del Atl{\'a}ntico, Barranquilla, Atl{\'a}ntico, Colombia}
\affiliation[11]{Augustana University, Sioux Falls, SD 57197, USA}
\affiliation[12]{University of Basel, CH-4056 Basel, Switzerland}
\affiliation[13]{University of Bern, CH-3012 Bern, Switzerland}
\affiliation[14]{Beykent University, Istanbul, Turkey}
\affiliation[15]{University of Birmingham, Birmingham B15 2TT, United Kingdom}
\affiliation[16]{Universit{\`a} del Bologna, 40127 Bologna, Italy}
\affiliation[17]{Boston University, Boston, MA 02215, USA}
\affiliation[18]{University of Bristol, Bristol BS8 1TL, United Kingdom}
\affiliation[19]{Brookhaven National Laboratory, Upton, NY 11973, USA}
\affiliation[20]{University of Bucharest, Bucharest, Romania}
\affiliation[21]{University of California Berkeley, Berkeley, CA 94720, USA}
\affiliation[22]{University of California Davis, Davis, CA 95616, USA}
\affiliation[23]{University of California Irvine, Irvine, CA 92697, USA}
\affiliation[24]{University of California Los Angeles, Los Angeles, CA 90095, USA}
\affiliation[25]{University of California Riverside, Riverside CA 92521, USA}
\affiliation[26]{University of California Santa Barbara, Santa Barbara, California 93106 USA}
\affiliation[27]{California Institute of Technology, Pasadena, CA 91125, USA}
\affiliation[28]{University of Cambridge, Cambridge CB3 0HE, United Kingdom}
\affiliation[29]{Universidade Estadual de Campinas, Campinas - SP, 13083-970, Brazil}
\affiliation[30]{Universit{\`a} di Catania, 2 - 95131 Catania, Italy}
\affiliation[31]{Universidad Cat{\'o}lica del Norte, Antofagasta, Chile}
\affiliation[32]{Centro Brasileiro de Pesquisas F\'isicas, Rio de Janeiro, RJ 22290-180, Brazil}
\affiliation[33]{IRFU, CEA, Universit{\'e} Paris-Saclay, F-91191 Gif-sur-Yvette, France}
\affiliation[34]{CERN, The European Organization for Nuclear Research, 1211 Meyrin, Switzerland}
\affiliation[35]{Institute of Particle and Nuclear Physics of the Faculty of Mathematics and Physics of the Charles University, 180 00 Prague 8, Czech Republic }
\affiliation[36]{University of Chicago, Chicago, IL 60637, USA}
\affiliation[37]{Chung-Ang University, Seoul 06974, South Korea}
\affiliation[38]{CIEMAT, Centro de Investigaciones Energ{\'e}ticas, Medioambientales y Tecnol{\'o}gicas, E-28040 Madrid, Spain}
\affiliation[39]{University of Cincinnati, Cincinnati, OH 45221, USA}
\affiliation[40]{Centro de Investigaci{\'o}n y de Estudios Avanzados del Instituto Polit{\'e}cnico Nacional (Cinvestav), Mexico City, Mexico}
\affiliation[41]{Universidad de Colima, Colima, Mexico}
\affiliation[42]{University of Colorado Boulder, Boulder, CO 80309, USA}
\affiliation[43]{Colorado State University, Fort Collins, CO 80523, USA}
\affiliation[44]{Columbia University, New York, NY 10027, USA}
\affiliation[45]{Comisi{\'o}n Nacional de Investigaci{\'o}n y Desarrollo Aeroespacial, Lima, Peru}
\affiliation[46]{Centro de Tecnologia da Informacao Renato Archer, Amarais - Campinas, SP - CEP 13069-901}
\affiliation[47]{Central University of South Bihar, Gaya, 824236, India }
\affiliation[48]{Institute of Physics, Czech Academy of Sciences, 182 00 Prague 8, Czech Republic}
\affiliation[49]{Czech Technical University, 115 19 Prague 1, Czech Republic}
\affiliation[50]{Dakota State University, Madison, SD 57042, USA}
\affiliation[51]{University of Dallas, Irving, TX 75062-4736, USA}
\affiliation[52]{Laboratoire d{\textquoteright}Annecy de Physique des Particules, Univ. Grenoble Alpes, Univ. Savoie Mont Blanc, CNRS, LAPP-IN2P3, 74000 Annecy, France}
\affiliation[53]{Daresbury Laboratory, Cheshire WA4 4AD, United Kingdom}
\affiliation[54]{Dordt University, 700 7th St NE, Sioux Center, IA 51250, USA}
\affiliation[55]{Drexel University, Philadelphia, PA 19104, USA}
\affiliation[56]{Duke University, Durham, NC 27708, USA}
\affiliation[57]{Durham University, Durham DH1 3LE, United Kingdom}
\affiliation[58]{University of Edinburgh, Edinburgh EH8 9YL, United Kingdom}
\affiliation[59]{Universidad EIA, Envigado, Antioquia, Colombia}
\affiliation[60]{E{\"o}tv{\"o}s Lor{\'a}nd University, 1053 Budapest, Hungary}
\affiliation[61]{ETH Zurich, Zurich, Switzerland}
\affiliation[62]{Faculdade de Ci{\^e}ncias da Universidade de Lisboa - FCUL, 1749-016 Lisboa, Portugal}
\affiliation[63]{Universidade Federal de Alfenas, Po{\c{c}}os de Caldas - MG, 37715-400, Brazil}
\affiliation[64]{Universidade Federal de Goias, Goiania, GO 74690-900, Brazil}
\affiliation[65]{Universidade Federal do ABC, Santo Andr{\'e} - SP, 09210-580, Brazil}
\affiliation[66]{Universidade Federal do Rio de Janeiro,  Rio de Janeiro - RJ, 21941-901, Brazil}
\affiliation[67]{Fermi National Accelerator Laboratory, Batavia, IL 60510, USA}
\affiliation[68]{University of Ferrara, Ferrara, Italy}
\affiliation[69]{University of Florida, Gainesville, FL 32611-8440, USA}
\affiliation[70]{Florida State University, Tallahassee, FL, USA}
\affiliation[71]{Fluminense Federal University, 9 Icara{\'\i} Niter{\'o}i - RJ, 24220-900, Brazil }
\affiliation[72]{Universit{\`a} degli Studi di Genova, Genova, Italy}
\affiliation[73]{Georgian Technical University, Tbilisi, Georgia}
\affiliation[74]{University of Granada {\&} CAFPE, 18002 Granada, Spain}
\affiliation[75]{Gran Sasso Science Institute, L'Aquila, Italy}
\affiliation[76]{Laboratori Nazionali del Gran Sasso, L'Aquila AQ, Italy}
\affiliation[77]{University Grenoble Alpes, CNRS, Grenoble INP, LPSC-IN2P3, 38000 Grenoble, France}
\affiliation[78]{Universidad de Guanajuato, Guanajuato, C.P. 37000, Mexico}
\affiliation[79]{Harish-Chandra Research Institute, Jhunsi, Allahabad 211 019, India}
\affiliation[80]{Harvard University, Cambridge, MA 02138, USA}
\affiliation[81]{University of Hawaii, Honolulu, HI 96822, USA}
\affiliation[82]{University of Houston, Houston, TX 77204, USA}
\affiliation[83]{University of  Hyderabad, Gachibowli, Hyderabad - 500 046, India}
\affiliation[84]{Idaho State University, Pocatello, ID 83209, USA}
\affiliation[85]{Institut de F{\'\i}sica d{\textquoteright}Altes Energies (IFAE){\textemdash}Barcelona Institute of Science and Technology (BIST), Barcelona, Spain}
\affiliation[86]{Instituto de F{\'\i}sica Corpuscular, CSIC and Universitat de Val{\`e}ncia, 46980 Paterna, Valencia, Spain}
\affiliation[87]{Instituto Galego de F{\'\i}sica de Altas Enerx{\'\i}as, University of Santiago de Compostela, 15782 Santiago de Compostela, Spain}
\affiliation[88]{Illinois Institute of Technology, Chicago, IL 60616, USA}
\affiliation[89]{Imperial College of Science Technology and Medicine, London SW7 2BZ, United Kingdom}
\affiliation[90]{Indian Institute of Technology Guwahati, Guwahati, 781 039, India}
\affiliation[91]{Indian Institute of Technology Hyderabad, Hyderabad, 502285, India}
\affiliation[92]{Indiana University, Bloomington, IN 47405, USA}
\affiliation[93]{Istituto Nazionale di Fisica Nucleare Sezione di Bologna, 40127 Bologna BO, Italy}
\affiliation[94]{Istituto Nazionale di Fisica Nucleare Sezione di Catania, I-95123 Catania, Italy}
\affiliation[95]{Istituto Nazionale di Fisica Nucleare Sezione di Ferrara, I-44122 Ferrara, Italy}
\affiliation[96]{Istituto Nazionale di Fisica Nucleare Laboratori Nazionali di Frascati, Frascati, Roma, Italy}
\affiliation[97]{Istituto Nazionale di Fisica Nucleare Sezione di Genova, 16146 Genova GE, Italy}
\affiliation[98]{Istituto Nazionale di Fisica Nucleare Sezione di Lecce, 73100 - Lecce, Italy}
\affiliation[99]{Istituto Nazionale di Fisica Nucleare Sezione di Milano Bicocca, 3 - I-20126 Milano, Italy}
\affiliation[100]{Istituto Nazionale di Fisica Nucleare Sezione di Milano, 20133 Milano, Italy}
\affiliation[101]{Istituto Nazionale di Fisica Nucleare Sezione di Napoli, I-80126 Napoli, Italy}
\affiliation[102]{Istituto Nazionale di Fisica Nucleare Sezione di Padova, 35131 Padova, Italy}
\affiliation[103]{Istituto Nazionale di Fisica Nucleare Sezione di Pavia,  I-27100 Pavia, Italy}
\affiliation[104]{Istituto Nazionale di Fisica Nucleare Laboratori Nazionali di Pisa, Pisa PI, Italy}
\affiliation[105]{Istituto Nazionale di Fisica Nucleare Sezione di Roma, 00185 Roma RM, Italy}
\affiliation[106]{Istituto Nazionale di Fisica Nucleare Laboratori Nazionali del Sud, 95123 Catania, Italy}
\affiliation[107]{Universidad Nacional de Ingenier{\'\i}a, Lima 25, Per{\'u}}
\affiliation[108]{Institute for Nuclear Research of the Russian Academy of Sciences, Moscow 117312, Russia}
\affiliation[109]{University of Insubria, Via Ravasi, 2, 21100 Varese VA, Italy}
\affiliation[110]{University of Iowa, Iowa City, IA 52242, USA}
\affiliation[111]{Iowa State University, Ames, Iowa 50011, USA}
\affiliation[112]{Institut de Physique des 2 Infinis de Lyon, 69622 Villeurbanne, France}
\affiliation[113]{Institute for Research in Fundamental Sciences, Tehran, Iran}
\affiliation[114]{Instituto Superior T{\'e}cnico - IST, Universidade de Lisboa, Portugal}
\affiliation[115]{Instituto Tecnol{\'o}gico de Aeron{\'a}utica, Sao Jose dos Campos, Brazil}
\affiliation[116]{Iwate University, Morioka, Iwate 020-8551, Japan}
\affiliation[117]{Jackson State University, Jackson, MS 39217, USA}
\affiliation[118]{University of Jammu, Jammu-180006, India}
\affiliation[119]{Jawaharlal Nehru University, New Delhi 110067, India}
\affiliation[120]{Jeonbuk National University, Jeonrabuk-do 54896, South Korea}
\affiliation[121]{Joint Institute for Nuclear Research, Dzhelepov Laboratory of Nuclear Problems 6 Joliot-Curie, Dubna, Moscow Region, 141980 RU }
\affiliation[122]{University of Jyvaskyla, FI-40014, Finland}
\affiliation[123]{Kansas State University, Manhattan, KS 66506, USA}
\affiliation[124]{Kavli Institute for the Physics and Mathematics of the Universe, Kashiwa, Chiba 277-8583, Japan}
\affiliation[125]{High Energy Accelerator Research Organization (KEK), Ibaraki, 305-0801, Japan}
\affiliation[126]{Korea Institute of Science and Technology Information, Daejeon, 34141, South Korea}
\affiliation[127]{K L University, Vaddeswaram, Andhra Pradesh 522502, India}
\affiliation[128]{National Institute of Technology, Kure College, Hiroshima, 737-8506, Japan}
\affiliation[129]{Taras Shevchenko National University of Kyiv, 01601 Kyiv, Ukraine}
\affiliation[130]{Lancaster University, Lancaster LA1 4YB, United Kingdom}
\affiliation[131]{Lawrence Berkeley National Laboratory, Berkeley, CA 94720, USA}
\affiliation[132]{Laborat{\'o}rio de Instrumenta{\c{c}}{\~a}o e F{\'\i}sica Experimental de Part{\'\i}culas, 1649-003 Lisboa and 3004-516 Coimbra, Portugal}
\affiliation[133]{University of Liverpool, L69 7ZE, Liverpool, United Kingdom}
\affiliation[134]{Los Alamos National Laboratory, Los Alamos, NM 87545, USA}
\affiliation[135]{Louisiana State University, Baton Rouge, LA 70803, USA}
\affiliation[136]{University of Lucknow, Uttar Pradesh 226007, India}
\affiliation[137]{Madrid Autonoma University and IFT UAM/CSIC, 28049 Madrid, Spain}
\affiliation[138]{Johannes Gutenberg-Universit{\"a}t Mainz, 55122 Mainz, Germany}
\affiliation[139]{University of Manchester, Manchester M13 9PL, United Kingdom}
\affiliation[140]{Massachusetts Institute of Technology, Cambridge, MA 02139, USA}
\affiliation[141]{Max-Planck-Institut, Munich, 80805, Germany}
\affiliation[142]{University of Medell{\'\i}n, Medell{\'\i}n, 050026 Colombia }
\affiliation[143]{University of Michigan, Ann Arbor, MI 48109, USA}
\affiliation[144]{Michigan State University, East Lansing, MI 48824, USA}
\affiliation[145]{Universit{\`a} del Milano-Bicocca, 20126 Milano, Italy}
\affiliation[146]{Universit{\`a} degli Studi di Milano, I-20133 Milano, Italy}
\affiliation[147]{University of Minnesota Duluth, Duluth, MN 55812, USA}
\affiliation[148]{University of Minnesota Twin Cities, Minneapolis, MN 55455, USA}
\affiliation[149]{University of Mississippi, University, MS 38677 USA}
\affiliation[150]{Universit{\`a} degli Studi di Napoli Federico II , 80138 Napoli NA, Italy}
\affiliation[151]{University of New Mexico, Albuquerque, NM 87131, USA}
\affiliation[152]{H. Niewodnicza{\'n}ski Institute of Nuclear Physics, Polish Academy of Sciences, Cracow, Poland}
\affiliation[153]{Nikhef National Institute of Subatomic Physics, 1098 XG Amsterdam, Netherlands}
\affiliation[154]{National Institute of Science Education and Research (NISER), Odisha 752050, India}
\affiliation[155]{University of North Dakota, Grand Forks, ND 58202-8357, USA}
\affiliation[156]{Northern Illinois University, DeKalb, IL 60115, USA}
\affiliation[157]{Northwestern University, Evanston, Il 60208, USA}
\affiliation[158]{University of Notre Dame, Notre Dame, IN 46556, USA}
\affiliation[159]{University of Novi Sad, 21102 Novi Sad, Serbia}
\affiliation[160]{Occidental College, Los Angeles, CA  90041}
\affiliation[161]{Ohio State University, Columbus, OH 43210, USA}
\affiliation[162]{Oregon State University, Corvallis, OR 97331, USA}
\affiliation[163]{University of Oxford, Oxford, OX1 3RH, United Kingdom}
\affiliation[164]{Pacific Northwest National Laboratory, Richland, WA 99352, USA}
\affiliation[165]{Universt{\`a} degli Studi di Padova, I-35131 Padova, Italy}
\affiliation[166]{Panjab University, Chandigarh, 160014 U.T., India}
\affiliation[167]{Universit{\'e} Paris-Saclay, CNRS/IN2P3, IJCLab, 91405 Orsay, France}
\affiliation[168]{Universit{\'e} Paris Cit{\'e}, CNRS, Astroparticule et Cosmologie, Paris, France}
\affiliation[169]{University of Parma,  43121 Parma PR, Italy}
\affiliation[170]{Universit{\`a} degli Studi di Pavia, 27100 Pavia PV, Italy}
\affiliation[171]{University of Pennsylvania, Philadelphia, PA 19104, USA}
\affiliation[172]{Pennsylvania State University, University Park, PA 16802, USA}
\affiliation[173]{Physical Research Laboratory, Ahmedabad 380 009, India}
\affiliation[174]{Universit{\`a} di Pisa, I-56127 Pisa, Italy}
\affiliation[175]{University of Pittsburgh, Pittsburgh, PA 15260, USA}
\affiliation[176]{Pontificia Universidad Cat{\'o}lica del Per{\'u}, Lima, Per{\'u}}
\affiliation[177]{University of Puerto Rico, Mayaguez 00681, Puerto Rico, USA}
\affiliation[178]{Punjab Agricultural University, Ludhiana 141004, India}
\affiliation[179]{Queen Mary University of London, London E1 4NS, United Kingdom }
\affiliation[180]{Radboud University, NL-6525 AJ Nijmegen, Netherlands}
\affiliation[181]{University of Rochester, Rochester, NY 14627, USA}
\affiliation[182]{Royal Holloway College London, TW20 0EX, United Kingdom}
\affiliation[183]{Rutgers University, Piscataway, NJ, 08854, USA}
\affiliation[184]{STFC Rutherford Appleton Laboratory, Didcot OX11 0QX, United Kingdom}
\affiliation[185]{Universit{\`a} del Salento, 73100 Lecce, Italy}
\affiliation[186]{San Jose State University, San Jos{\'e}, CA 95192-0106, USA}
\affiliation[187]{Sapienza University of Rome, 00185 Roma RM, Italy}
\affiliation[188]{Universidad Sergio Arboleda, 11022 Bogot{\'a}, Colombia}
\affiliation[189]{University of Sheffield, Sheffield S3 7RH, United Kingdom}
\affiliation[190]{SLAC National Accelerator Laboratory, Menlo Park, CA 94025, USA}
\affiliation[191]{University of South Carolina, Columbia, SC 29208, USA}
\affiliation[192]{South Dakota School of Mines and Technology, Rapid City, SD 57701, USA}
\affiliation[193]{South Dakota State University, Brookings, SD 57007, USA}
\affiliation[194]{Southern Methodist University, Dallas, TX 75275, USA}
\affiliation[195]{Stony Brook University, SUNY, Stony Brook, NY 11794, USA}
\affiliation[196]{Sun Yat-Sen University, Guangzhou, 510275}
\affiliation[197]{Sanford Underground Research Facility, Lead, SD, 57754, USA}
\affiliation[198]{University of Sussex, Brighton, BN1 9RH, United Kingdom}
\affiliation[199]{Syracuse University, Syracuse, NY 13244, USA}
\affiliation[200]{Universidade Tecnol{\'o}gica Federal do Paran{\'a}, Curitiba, Brazil}
\affiliation[201]{Tel Aviv University, Tel Aviv-Yafo, Israel}
\affiliation[202]{Texas A{\&}M University, College Station, Texas 77840}
\affiliation[203]{Texas A{\&}M University - Corpus Christi, Corpus Christi, TX 78412, USA}
\affiliation[204]{University of Texas at Arlington, Arlington, TX 76019, USA}
\affiliation[205]{University of Texas at Austin, Austin, TX 78712, USA}
\affiliation[206]{University of Toronto, Toronto, Ontario M5S 1A1, Canada}
\affiliation[207]{Tufts University, Medford, MA 02155, USA}
\affiliation[208]{Universidade Federal de S{\~a}o Paulo, 09913-030, S{\~a}o Paulo, Brazil}
\affiliation[209]{Ulsan National Institute of Science and Technology, Ulsan 689-798, South Korea}
\affiliation[210]{University College London, London, WC1E 6BT, United Kingdom}
\affiliation[211]{Valley City State University, Valley City, ND 58072, USA}
\affiliation[212]{Variable Energy Cyclotron Centre, 700 064 West Bengal, India}
\affiliation[213]{Virginia Tech, Blacksburg, VA 24060, USA}
\affiliation[214]{University of Warsaw, 02-093 Warsaw, Poland}
\affiliation[215]{University of Warwick, Coventry CV4 7AL, United Kingdom}
\affiliation[216]{Wellesley College, Wellesley, MA 02481, USA}
\affiliation[217]{Wichita State University, Wichita, KS 67260, USA}
\affiliation[218]{William and Mary, Williamsburg, VA 23187, USA}
\affiliation[219]{University of Wisconsin Madison, Madison, WI 53706, USA}
\affiliation[220]{Yale University, New Haven, CT 06520, USA}
\affiliation[221]{Yerevan Institute for Theoretical Physics and Modeling, Yerevan 0036, Armenia}
\affiliation[222]{York University, Toronto M3J 1P3, Canada}
%----------------------------------------------------
% Authors in alphabetical order
\author[34]{A.~Abed Abud,}
\author[163]{B.~Abi,}
\author[67]{R.~Acciarri,}
\author[10]{M.~A.~Acero,}
\author[200]{M.~R.~Adames,}
\author[73]{G.~Adamov,}
\author[67]{M.~Adamowski,}
\author[19]{D.~Adams,}
\author[18]{M.~Adinolfi,}
\author[29]{C.~Adriano,}
\author[82]{A.~Aduszkiewicz,}
\author[131]{J.~Aguilar,}
\author[212]{Z.~Ahmad,}
\author[215]{J.~Ahmed,}
\author[52]{B.~Aimard,}
\author[181]{F.~Akbar,}
\author[42]{K.~Allison,}
\author[34]{S.~Alonso Monsalve,}
\author[123]{M.~Alrashed,}
\author[61]{C.~Alt,}
\author[11]{A.~Alton,}
\author[38]{R.~Alvarez,}
\author[87,86]{P.~Amedo,}
\author[6]{J.~Anderson,}
\author[88]{D. A. ~Andrade,}
\author[184,133]{C.~Andreopoulos,}
\author[95,68]{M.~Andreotti,}
\author[67]{M.~P.~Andrews,}
\author[4]{F.~Andrianala,}
\author[132]{S.~Andringa,}
\author[121]{N.~Anfimov,}
\author[63]{W.~L.~Anic{\'e}zio Campanelli,}
\author[190]{A.~Ankowski,}
\author[200]{M.~Antoniassi,}
\author[86]{M.~Antonova,}
\author[121]{A.~Antoshkin,}
\author[12]{S.~Antusch,}
\author[41]{A.~Aranda-Fernandez,}
\author[139]{L.~Arellano,}
\author[44]{L.~O.~Arnold,}
\author[59]{M.~A.~Arroyave,}
\author[204]{J.~Asaadi,}
\author[201]{A.~Ashkenazi,}
\author[198]{L.~Asquith,}
\author[39]{A.~Aurisano,}
\author[129]{V.~Aushev,}
\author[112]{D.~Autiero,}
\author[40]{M.~Ayala-Torres,}
\author[163]{F.~Azfar,}
\author[92]{A.~Back,}
\author[164]{H.~Back,}
\author[215]{J.~J.~Back,}
\author[73]{I.~Bagaturia,}
\author[67]{L.~Bagby,}
\author[121]{N.~Balashov,}
\author[67]{S.~Balasubramanian,}
\author[23]{P.~Baldi,}
\author[95]{W.~Baldini,}
\author[67]{B.~Baller,}
\author[83]{B.~Bambah,}
\author[132,114]{F.~Barao,}
\author[86]{G.~Barenboim,}
\author[34]{P.\ Barham~Alz\'as,}
\author[215]{G.~J.~Barker,}
\author[155]{W.~Barkhouse,}
\author[143]{C.~Barnes,}
\author[163]{G.~Barr,}
\author[78]{J.~Barranco Monarca,}
\author[200]{A.~Barros,}
\author[132,62]{N.~Barros,}
\author[140]{J.~L.~Barrow,}
\author[210]{A.~Basharina-Freshville,}
\author[6]{A.~Bashyal,}
\author[67]{V.~Basque,}
\author[58]{C.~Batchelor,}
\author[216]{J.B.R.~Battat,}
\author[163]{F.~Battisti,}
\author[3]{F.~Bay,}
\author[29]{M.~C.~Q.~Bazetto,}
\author[176]{J.~L.~L.~Bazo Alba,}
\author[161]{J.~F.~Beacom,}
\author[112]{E.~Bechetoille,}
\author[43]{B.~Behera,}
\author[29]{E.~Belchior,}
\author[67]{L.~Bellantoni,}
\author[104,174]{G.~Bellettini,}
\author[94,30]{V.~Bellini,}
\author[34]{O.~Beltramello,}
\author[34]{N.~Benekos,}
\author[8]{C.~Benitez Montiel,}
\author[19]{D.~Benjamin,}
\author[132]{F.~Bento Neves,}
\author[43]{J.~Berger,}
\author[67]{S.~Berkman,}
\author[98,185]{P.~Bernardini,}
\author[13]{R.~M.~Berner,}
\author[97]{A.~Bersani,}
\author[93,16]{S.~Bertolucci,}
\author[67]{M.~Betancourt,}
\author[59]{A.~Betancur Rodr\'iguez,}
\author[179]{A.~Bevan,}
\author[22]{Y.~Bezawada,}
\author[63]{A.~T.~Bezerra,}
\author[198]{T.~J.~Bezerra,}
\author[195]{J.~Bhambure,}
\author[135]{A.~Bhardwaj,}
\author[166]{V.~Bhatnagar,}
\author[90]{M.~Bhattacharjee,}
\author[67]{M.~Bhattacharya,}
\author[149]{D.~Bhattarai,}
\author[18]{S.~Bhuller,}
\author[90]{B.~Bhuyan,}
\author[106]{S.~Biagi,}
\author[23]{J.~Bian,}
\author[99]{M.~Biassoni,}
\author[67]{K.~Biery,}
\author[14,110]{B.~Bilki,}
\author[19]{M.~Bishai,}
\author[101]{V.~Bisignani,}
\author[139]{A.~Bitadze,}
\author[130]{A.~Blake,}
\author[67]{F.~D.~Blaszczyk,}
\author[156]{G.~C.~Blazey,}
\author[110]{D.~Blend,}
\author[36]{E.~Blucher,}
\author[134]{J.~Boissevain,}
\author[33]{S.~Bolognesi,}
\author[123]{T.~Bolton,}
\author[99,109]{L.~Bomben,}
\author[99,145]{M.~Bonesini,}
\author[31]{C.~Bonilla-Diaz,}
\author[19]{F.~Bonini,}
\author[179]{A.~Booth,}
\author[14]{F.~Boran,}
\author[34]{S.~Bordoni,}
\author[198]{A.~Borkum,}
\author[110]{N.~Bostan,}
\author[49]{P.~Bour,}
\author[156]{D.~Boyden,}
\author[15]{J.~Bracinik,}
\author[67]{D.~Braga,}
\author[130]{D.~Brailsford,}
\author[99]{A.~Branca,}
\author[204]{A.~Brandt,}
\author[74]{M.~Bravo-Moreno,}
\author[34]{J.~Bremer,}
\author[184]{C.~Brew,}
\author[67]{S.~J.~Brice,}
\author[99,145]{C.~Brizzolari,}
\author[144]{C.~Bromberg,}
\author[18]{J.~Brooke,}
\author[67]{A.~Bross,}
\author[99,145]{G.~Brunetti,}
\author[215]{M.~Brunetti,}
\author[43]{N.~Buchanan,}
\author[181]{H.~Budd,}
\author[13]{J.~Buergi,}
\author[22]{G.~Caceres V.,}
\author[93,16]{I.~Cagnoli,}
\author[222]{T.~Cai,}
\author[112]{D.~Caiulo,}
\author[95,68]{R.~Calabrese,}
\author[131]{P.~Calafiura,}
\author[162]{J.~Calcutt,}
\author[20]{M.~Calin,}
\author[13]{L.~Calivers,}
\author[43]{S.~Calvez,}
\author[38]{E.~Calvo,}
\author[97]{A.~Caminata,}
\author[26]{D.~Caratelli,}
\author[43]{D.~Carber,}
\author[210]{J.~C.~Carceller,}
\author[19]{G.~Carini,}
\author[112]{B.~Carlus,}
\author[19]{M.~F.~Carneiro,}
\author[99]{P.~Carniti,}
\author[43]{I.~Caro Terrazas,}
\author[204]{H.~Carranza,}
\author[22]{N.~Carrara,}
\author[123]{L.~Carroll,}
\author[219]{T.~Carroll,}
\author[182]{A.~Carter,}
\author[5]{J.~F.~Casta{\~n}o Forero,}
\author[188]{A.~Castillo,}
\author[218]{E.~Catano-Mur,}
\author[99]{C.~Cattadori,}
\author[167]{F.~Cavalier,}
\author[99]{G.~Cavallaro,}
\author[67]{F.~Cavanna,}
\author[165]{S.~Centro,}
\author[67]{G.~Cerati,}
\author[93]{A.~Cervelli,}
\author[86]{A.~Cervera Villanueva,}
\author[173]{K.~Chakraborty,}
\author[34]{M.~Chalifour,}
\author[215]{A.~Chappell,}
\author[168]{E.~Chardonnet,}
\author[34]{N.~Charitonidis,}
\author[175]{A.~Chatterjee,}
\author[212]{S.~Chattopadhyay,}
\author[19]{H.~Chen,}
\author[23]{M.~Chen,}
\author[13,190]{Y.~Chen,}
\author[195]{Z.~Chen,}
\author[182]{Z.~Chen-Wishart,}
\author[209]{Y.~Cheon,}
\author[82]{D.~Cherdack,}
\author[44]{C.~Chi,}
\author[67]{S.~Childress,}
\author[88]{R.~Chirco,}
\author[20]{A.~Chiriacescu,}
\author[104,174]{N.~Chitirasreemadam,}
\author[126]{K.~Cho,}
\author[156]{S.~Choate,}
\author[73]{D.~Chokheli,}
\author[171]{P.~S.~Chong,}
\author[6]{B.~Chowdhury,}
\author[43]{A.~Christensen,}
\author[67]{D.~Christian,}
\author[34]{G.~Christodoulou,}
\author[121]{A.~Chukanov,}
\author[209]{M.~Chung,}
\author[164]{E.~Church,}
\author[93,16]{V.~Cicero,}
\author[214]{D.~Clapa,}
\author[58]{P.~Clarke,}
\author[131]{G.~Cline,}
\author[194]{T.~E.~Coan,}
\author[101]{A.~G.~Cocco,}
\author[168]{J.~A.~B.~Coelho,}
\author[168]{A.~Cohen,}
\author[77]{J.~Collot,}
\author[56]{E.~Conley,}
\author[140]{J.~M.~Conrad,}
\author[190]{M.~Convery,}
\author[97]{S.~Copello,}
\author[100,169]{P.~Cova,}
\author[182]{C.~Cox,}
\author[149]{L.~Cremaldi,}
\author[179]{L.~Cremonesi,}
\author[38]{J.~I.~Crespo-Anad\'on,}
\author[67]{M.~Crisler,}
\author[100,8]{E.~Cristaldo,}
\author[67]{J.~Crnkovic,}
\author[210]{G.~Crone,}
\author[130]{R.~Cross,}
\author[42]{A.~Cudd,}
\author[38]{C.~Cuesta,}
\author[25]{Y.~Cui,}
\author[18]{D.~Cussans,}
\author[77]{J.~Dai,}
\author[23]{O.~Dalager,}
\author[168]{R.~Dallavalle,}
\author[32]{H.~da Motta,}
\author[218]{Z.~A.~Dar,}
\author[198]{R.~Darby,}
\author[66]{L.~Da Silva Peres,}
\author[222,67]{C.~David,}
\author[112]{Q.~David,}
\author[149]{G.~S.~Davies,}
\author[97]{S.~Davini,}
\author[168]{J.~Dawson,}
\author[204]{K.~De,}
\author[1]{S.~De,}
\author[29]{R.~De Aguiar,}
\author[29]{P.~De Almeida,}
\author[110]{P.~Debbins,}
\author[52]{I.~De Bonis,}
\author[153,2]{M.~P.~Decowski,}
\author[157]{A.~de Gouv\^ea,}
\author[29]{P.~C.~De Holanda,}
\author[198]{I.~L.~De Icaza Astiz,}
\author[138]{A.~Deisting,}
\author[153,2]{P.~De Jong,}
\author[38]{A.~De la Torre,}
\author[33]{A.~Delbart,}
\author[187,105]{V.~De Leo,}
\author[78]{D.~Delepine,}
\author[99,145]{M.~Delgado,}
\author[34]{A.~Dell'Acqua,}
\author[100,169]{N.~Delmonte,}
\author[6]{P.~De Lurgio,}
\author[66]{J.~R.~T.~de Mello Neto,}
\author[211]{D.~M.~DeMuth,}
\author[28]{S.~Dennis,}
\author[184]{C.~Densham,}
\author[19]{P.~Denton,}
\author[19]{G.~W.~Deptuch,}
\author[34]{A.~De Roeck,}
\author[86]{V.~De Romeri,}
\author[29]{G.~De Souza,}
\author[28]{J.~P.~Detje,}
\author[118]{R.~Devi,}
\author[81]{R.~Dharmapalan,}
\author[208]{M.~Dias,}
\author[92]{J.~S.~D\'iaz,}
\author[176]{F.~D{\'\i}az,}
\author[101,150]{F.~Di Capua,}
\author[187,105]{A.~Di Domenico,}
\author[97,72]{S.~Di Domizio,}
\author[104]{S.~Di Falco,}
\author[34]{L.~Di Giulio,}
\author[67]{P.~Ding,}
\author[97,72]{L.~Di Noto,}
\author[96]{E.~Diociaiuti,}
\author[106]{C.~Distefano,}
\author[13]{R.~Diurba,}
\author[19]{M.~Diwan,}
\author[6]{Z.~Djurcic,}
\author[190]{D.~Doering,}
\author[34]{S.~Dolan,}
\author[14]{F.~Dolek,}
\author[55]{M.~J.~Dolinski,}
\author[96]{D.~Domenici,}
\author[190]{L.~Domine,}
\author[104,174]{S.~Donati,}
\author[34]{Y.~Donon,}
\author[111]{S.~Doran,}
\author[144]{D.~Douglas,}
\author[190]{A.~Dragone,}
\author[190]{F.~Drielsma,}
\author[208]{L.~Duarte,}
\author[52]{D.~Duchesneau,}
\author[163,67]{K.~Duffy,}
\author[23]{K.~Dugas,}
\author[89]{P.~Dunne,}
\author[202]{B.~Dutta,}
\author[191]{H.~Duyang,}
\author[81]{O.~Dvornikov,}
\author[131]{D.~A.~Dwyer,}
\author[156]{A.~S.~Dyshkant,}
\author[156]{M.~Eads,}
\author[198]{A.~Earle,}
\author[144]{D.~Edmunds,}
\author[67]{J.~Eisch,}
\author[139,141]{L.~Emberger,}
\author[183]{P.~Englezos,}
\author[220]{A.~Ereditato,}
\author[22]{T.~Erjavec,}
\author[67]{C.~O.~Escobar,}
\author[139]{J.~J.~Evans,}
\author[92]{E.~Ewart,}
\author[189]{A.~C.~Ezeribe,}
\author[67]{K.~Fahey,}
\author[34]{L.~Fajt,}
\author[99,145]{A.~Falcone,}
\author[134]{M.~Fani',}
\author[102]{C.~Farnese,}
\author[113]{Y.~Farzan,}
\author[121]{D.~Fedoseev,}
\author[78]{J.~Felix,}
\author[111]{Y.~Feng,}
\author[137]{E.~Fernandez-Martinez,}
\author[97,72]{F.~Ferraro,}
\author[158]{L.~Fields,}
\author[48]{P.~Filip,}
\author[199]{A.~Filkins,}
\author[153,180]{F.~Filthaut,}
\author[134]{R.~Fine,}
\author[101,150]{G.~Fiorillo,}
\author[95,68]{M.~Fiorini,}
\author[111]{V.~Fischer,}
\author[143]{R.~S.~Fitzpatrick,}
\author[51]{W.~Flanagan,}
\author[36,220]{B.~Fleming,}
\author[181]{R.~Flight,}
\author[43]{S.~Fogarty,}
\author[88]{W.~Foreman,}
\author[56]{J.~Fowler,}
\author[49]{J.~Franc,}
\author[220]{D.~Franco,}
\author[67]{J.~Freeman,}
\author[19]{J.~Fried,}
\author[190]{A.~Friedland,}
\author[67]{S.~Fuess,}
\author[69]{I.~K.~Furic,}
\author[179]{K.~Furman,}
\author[148]{A.~P.~Furmanski,}
\author[93,16]{A.~Gabrielli,}
\author[176]{A.~Gago,}
\author[207]{H.~Gallagher,}
\author[167]{A.~Gallas,}
\author[38]{A.~Gallego-Ros,}
\author[100,146]{N.~Gallice,}
\author[112]{V.~Galymov,}
\author[34]{E.~Gamberini,}
\author[189]{T.~Gamble,}
\author[200]{F.~Ganacim,}
\author[79]{R.~Gandhi,}
\author[67]{S.~Ganguly,}
\author[175]{F.~Gao,}
\author[19]{S.~Gao,}
\author[74]{D.~Garcia-Gamez,}
\author[86]{M.~\'A.~Garc\'ia-Peris,}
\author[67]{S.~Gardiner,}
\author[17]{D.~Gastler,}
\author[13]{A.~Gauch,}
\author[160]{J.~Gauvreau,}
\author[187,105]{P.~Gauzzi,}
\author[44]{G.~Ge,}
\author[52]{N.~Geffroy,}
\author[29]{B.~Gelli,}
\author[61]{A.~Gendotti,}
\author[193]{S.~Gent,}
\author[19]{L.~Gerlach,}
\author[97]{Z.~Ghorbani-Moghaddam,}
\author[29]{P.~Giammaria,}
\author[95,68]{T.~Giammaria,}
\author[206]{N.~Giangiacomi,}
\author[165,102]{D.~Gibin,}
\author[38]{I.~Gil-Botella,}
\author[162]{S.~Gilligan,}
\author[104]{A.~Gioiosa,}
\author[96]{S.~Giovannella,}
\author[112]{C.~Girerd,}
\author[91]{A.~K.~Giri,}
\author[131]{D.~Gnani,}
\author[129]{O.~Gogota,}
\author[151]{M.~Gold,}
\author[134]{S.~Gollapinni,}
\author[67]{K.~Gollwitzer,}
\author[64]{R.~A.~Gomes,}
\author[188]{L.~V.~Gomez Bermeo,}
\author[188]{L.~S.~Gomez Fajardo,}
\author[15]{F.~Gonnella,}
\author[87]{D.~Gonzalez-Diaz,}
\author[137]{M.~Gonzalez-Lopez,}
\author[6]{M.~C.~Goodman,}
\author[139]{O.~Goodwin,}
\author[173]{S.~Goswami,}
\author[99]{C.~Gotti,}
\author[135]{J.~Goudeau,}
\author[15]{E.~Goudzovski,}
\author[131]{C.~Grace,}
\author[147]{R.~Gran,}
\author[78]{E.~Granados,}
\author[168]{P.~Granger,}
\author[17]{C.~Grant,}
\author[71]{D.~Gratieri,}
\author[163]{P.~Green,}
\author[21,131]{S.~Greenberg,}
\author[219]{L.~Greenler,}
\author[18]{J.~Greer,}
\author[34]{J.~Grenard,}
\author[198]{W.~C.~Griffith,}
\author[34]{F.~T.~Groetschla,}
\author[43]{M.~Groh,}
\author[214]{K.~Grzelak,}
\author[19]{W.~Gu,}
\author[6]{V.~Guarino,}
\author[95,68]{M.~Guarise,}
\author[139]{R.~Guenette,}
\author[167]{E.~Guerard,}
\author[93]{M.~Guerzoni,}
\author[99]{D.~Guffanti,}
\author[102]{A.~Guglielmi,}
\author[191]{B.~Guo,}
\author[190]{A.~Gupta,}
\author[153,2]{V.~Gupta,}
\author[127]{K.~K.~Guthikonda,}
\author[139]{P.~Guzowski,}
\author[29]{M.~M.~Guzzo,}
\author[37]{S.~Gwon,}
\author[37]{C.~Ha,}
\author[67]{K.~Haaf,}
\author[147]{A.~Habig,}
\author[204]{H.~Hadavand,}
\author[138]{A.~Hadef,}
\author[13]{R.~Haenni,}
\author[220]{L.~Hagaman,}
\author[67]{A.~Hahn,}
\author[192]{J.~Haiston,}
\author[163]{P.~Hamacher-Baumann,}
\author[67]{T.~Hamernik,}
\author[89]{P.~Hamilton,}
\author[175]{J.~Han,}
\author[15]{J.~Hancock,}
\author[96]{F.~Happacher,}
\author[222,67]{D.~A.~Harris,}
\author[198]{J.~Hartnell,}
\author[184]{T.~Hartnett,}
\author[43]{J.~Harton,}
\author[125]{T.~Hasegawa,}
\author[163]{C.~Hasnip,}
\author[67]{R.~Hatcher,}
\author[23]{K.~W.~Hatfield,}
\author[186]{A.~Hatzikoutelis,}
\author[92]{C.~Hayes,}
\author[179]{K.~Hayrapetyan,}
\author[179]{J.~Hays,}
\author[17]{E.~Hazen,}
\author[82]{M.~He,}
\author[67]{A.~Heavey,}
\author[220]{K.~M.~Heeger,}
\author[197]{J.~Heise,}
\author[181]{S.~Henry,}
\author[88]{M.~A.~Hernandez Morquecho,}
\author[67]{K.~Herner,}
\author[39]{V.~Hewes,}
\author[148]{C.~Hilgenberg,}
\author[84]{T.~Hill,}
\author[15]{S.~J.~Hillier,}
\author[67]{A.~Himmel,}
\author[36]{E.~Hinkle,}
\author[200]{L.R.~Hirsch,}
\author[54]{J.~Ho,}
\author[67]{J.~Hoff,}
\author[184]{A.~Holin,}
\author[163]{T.~Holvey,}
\author[164]{E.~Hoppe,}
\author[123]{G.~A.~Horton-Smith,}
\author[148]{M.~Hostert,}
\author[167]{T.~Houdy,}
\author[140]{A.~Hourlier,}
\author[67]{B.~Howard,}
\author[181]{R.~Howell,}
\author[142]{J.~Hoyos Barrios,}
\author[184]{I.~Hristova,}
\author[67]{M.~S.~Hronek,}
\author[22]{J.~Huang,}
\author[131]{R.G.~Huang,}
\author[190]{Z.~Hulcher,}
\author[89]{G.~Iles,}
\author[206]{N.~Ilic,}
\author[93]{A.~M.~Iliescu,}
\author[67]{R.~Illingworth,}
\author[93,16]{G.~Ingratta,}
\author[221]{A.~Ioannisian,}
\author[148]{B.~Irwin,}
\author[0]{L.~Isenhower,}
\author[66]{M.~Ismerio Oliveira,}
\author[190]{R.~Itay,}
\author[164]{C.M.~Jackson,}
\author[1]{V.~Jain,}
\author[67]{E.~James,}
\author[204]{W.~Jang,}
\author[23]{B.~Jargowsky,}
\author[49]{F.~Jediny,}
\author[67]{D.~Jena,}
\author[37]{Y.~S.~Jeong,}
\author[85]{C.~Jes\'{u}s-Valls,}
\author[19]{X.~Ji,}
\author[195]{J.~Jiang,}
\author[213]{L.~Jiang,}
\author[20]{A.~Jipa,}
\author[220]{J.~H.~Jo,}
\author[132,114]{F.~R.~Joaquim,}
\author[192]{W.~Johnson,}
\author[204]{B.~Jones,}
\author[189]{R.~Jones,}
\author[159]{N.~Jovancevic,}
\author[175]{M.~Judah,}
\author[195]{C.~K.~Jung,}
\author[67]{T.~Junk,}
\author[44]{Y.~Jwa,}
\author[89]{M.~Kabirnezhad,}
\author[182,184]{A.~Kaboth,}
\author[129]{I.~Kadenko,}
\author[121]{I.~Kakorin,}
\author[121]{A.~Kalitkina,}
\author[44]{D.~Kalra,}
\author[110]{O.~Kamer Koseyan,}
\author[65]{F.~Kamiya,}
\author[88]{D.~M.~Kaplan,}
\author[44]{G.~Karagiorgi,}
\author[110]{G.~Karaman,}
\author[131]{A.~Karcher,}
\author[52]{Y.~Karyotakis,}
\author[128]{S.~Kasai,}
\author[135]{S.~P.~Kasetti,}
\author[43]{L.~Kashur,}
\author[15]{I.~Katsioulas,}
\author[221]{N.~Kazaryan,}
\author[17]{E.~Kearns,}
\author[171]{P.~Keener,}
\author[34]{K.J.~Kelly,}
\author[29]{E.~Kemp,}
\author[73]{O.~Kemularia,}
\author[167]{Y.~Kermaidic,}
\author[67]{W.~Ketchum,}
\author[19]{S.~H.~Kettell,}
\author[108]{M.~Khabibullin,}
\author[108]{A.~Khotjantsev,}
\author[73]{A.~Khvedelidze,}
\author[202]{D.~Kim,}
\author[67]{B.~King,}
\author[44]{B.~Kirby,}
\author[67]{M.~Kirby,}
\author[171]{J.~Klein,}
\author[149]{J.~Kleykamp,}
\author[89]{A.~Klustova,}
\author[67]{T.~Kobilarcik,}
\author[219]{K.~Koehler,}
\author[82]{L.~W.~Koerner,}
\author[190]{D.~H.~Koh,}
\author[21,131]{S.~Kohn,}
\author[13]{P.~P.~Koller,}
\author[121]{L.~Kolupaeva,}
\author[121]{D.~Korablev,}
\author[218]{M.~Kordosky,}
\author[77]{T.~Kosc,}
\author[34]{U.~Kose,}
\author[92]{V.~A.~Kosteleck\'y,}
\author[18]{K.~Kothekar,}
\author[55]{I.~Kotler,}
\author[121]{V.~Kozhukalov,}
\author[198]{R.~Kralik,}
\author[18]{L.~Kreczko,}
\author[111]{F.~Krennrich,}
\author[13]{I.~Kreslo,}
\author[23]{W.~Kropp,}
\author[171]{T.~Kroupova,}
\author[34]{M.~Kubu,}
\author[108]{Y.~Kudenko,}
\author[189]{V.~A.~Kudryavtsev,}
\author[6]{S.~Kuhlmann,}
\author[108]{S.~Kulagin,}
\author[81]{J.~Kumar,}
\author[189]{P.~Kumar,}
\author[52]{P.~Kunze,}
\author[131]{R.~Kuravi,}
\author[190]{N.~Kurita,}
\author[191]{C.~Kuruppu,}
\author[49]{V.~Kus,}
\author[135]{T.~Kutter,}
\author[48]{J.~Kvasnicka,}
\author[209]{D.~Kwak,}
\author[131]{A.~Lambert,}
\author[171]{B.~J.~Land,}
\author[55]{C.~E.~Lane,}
\author[205]{K.~Lang,}
\author[220]{T.~Langford,}
\author[139]{M.~Langstaff,}
\author[34]{F.~Lanni,}
\author[52]{O.~Lantwin,}
\author[19]{J.~Larkin,}
\author[89]{P.~Lasorak,}
\author[171]{D.~Last,}
\author[219]{A.~Laundrie,}
\author[93]{G.~Laurenti,}
\author[131]{A.~Lawrence,}
\author[19]{P.~Laycock,}
\author[20]{I.~Lazanu,}
\author[100,146]{M.~Lazzaroni,}
\author[207]{T.~Le,}
\author[87]{S.~Leardini,}
\author[81]{J.~Learned,}
\author[112]{P.~LeBrun,}
\author[190]{T.~LeCompte,}
\author[67]{C.~Lee,}
\author[129]{V.~Legin,}
\author[34]{G.~Lehmann Miotto,}
\author[92]{R.~Lehnert,}
\author[65]{M.~A.~Leigui de Oliveira,}
\author[131]{M.~Leitner,}
\author[139]{L.~M.~Lepin,}
\author[190]{S.~W.~Li,}
\author[19]{Y.~Li,}
\author[123]{H.~Liao,}
\author[131]{C.~S.~Lin,}
\author[135]{S.~Lin,}
\author[18]{D.~Lindebaum,}
\author[31]{R.~A.~Lineros,}
\author[196]{J.~Ling,}
\author[219]{A.~Lister,}
\author[88]{B.~R.~Littlejohn,}
\author[23]{J.~Liu,}
\author[36]{Y.~Liu,}
\author[67]{S.~Lockwitz,}
\author[131]{T.~Loew,}
\author[48]{M.~Lokajicek,}
\author[73]{I.~Lomidze,}
\author[89]{K.~Long,}
\author[215]{T.~Lord,}
\author[158]{J.~M.~LoSecco,}
\author[134]{W.~C.~Louis,}
\author[215]{X.-G.~Lu,}
\author[21,131]{K.B.~Luk,}
\author[171]{B.~Lunday,}
\author[26]{X.~Luo,}
\author[95,68]{E.~Luppi,}
\author[85]{T.~Lux,}
\author[65]{V.~P.~Luzio,}
\author[167]{J.~Maalmi,}
\author[190]{D.~MacFarlane,}
\author[29]{A.~A.~Machado,}
\author[67]{P.~Machado,}
\author[92]{C.~T.~Macias,}
\author[67]{J.~R.~Macier,}
\author[210]{M.~MacMahon,}
\author[76]{A.~Maddalena,}
\author[34]{A.~Madera,}
\author[21,131]{P.~Madigan,}
\author[6]{S.~Magill,}
\author[144]{K.~Mahn,}
\author[132,62]{A.~Maio,}
\author[56]{A.~Major,}
\author[133]{K.~Majumdar,}
\author[50]{J.~A.~Maloney,}
\author[206]{M.~Man,}
\author[93]{G.~Mandrioli,}
\author[23]{R.~C.~Mandujano,}
\author[132,62]{J.~Maneira,}
\author[210]{L.~Manenti,}
\author[181]{S.~Manly,}
\author[207]{A.~Mann,}
\author[184]{K.~Manolopoulos,}
\author[92]{M.~Manrique Plata,}
\author[19]{V.~N.~Manyam,}
\author[67]{M.~Marchan,}
\author[67]{A.~Marchionni,}
\author[19]{W.~Marciano,}
\author[81]{D.~Marfatia,}
\author[213]{C.~Mariani,}
\author[81]{J.~Maricic,}
\author[115]{F.~Marinho,}
\author[42]{A.~D.~Marino,}
\author[190]{T.~Markiewicz,}
\author[139]{D.~Marsden,}
\author[148]{M.~Marshak,}
\author[181]{C.~M.~Marshall,}
\author[215]{J.~Marshall,}
\author[112]{J.~Marteau,}
\author[86]{J.~Mart{\'\i}n-Albo,}
\author[123]{N.~Martinez,}
\author[192]{D.A.~Martinez Caicedo ,}
\author[179]{F.~Mart{\'i}nez L{\'o}pez,}
\author[86]{P.~Mart\'inez Mirav\'e,}
\author[19]{S.~Martynenko,}
\author[99,109]{V.~Mascagna,}
\author[207]{K.~Mason,}
\author[183]{A.~Mastbaum,}
\author[131]{F.~Matichard,}
\author[81]{S.~Matsuno,}
\author[135]{J.~Matthews,}
\author[171]{C.~Mauger,}
\author[93,16]{N.~Mauri,}
\author[133]{K.~Mavrokoridis,}
\author[215]{I.~Mawby,}
\author[99]{R.~Mazza,}
\author[67]{A.~Mazzacane,}
\author[216]{T.~McAskill,}
\author[67]{E.~McCluskey,}
\author[210]{N.~McConkey,}
\author[181]{K.~S.~McFarland,}
\author[195]{C.~McGrew,}
\author[139]{A.~McNab,}
\author[108]{A.~Mefodiev,}
\author[119]{P.~Mehta,}
\author[9]{P.~Melas,}
\author[86]{O.~Mena,}
\author[177]{H.~Mendez,}
\author[34]{P.~Mendez,}
\author[19]{D.~P.~M{\'e}ndez,}
\author[103,170]{A.~Menegolli,}
\author[102]{G.~Meng,}
\author[92]{M.~D.~Messier,}
\author[135]{W.~Metcalf,}
\author[92]{M.~Mewes,}
\author[217]{H.~Meyer,}
\author[67]{T.~Miao,}
\author[193]{G.~Michna,}
\author[210]{V.~Mikola,}
\author[81]{R.~Milincic,}
\author[139]{G.~Miller,}
\author[148]{W.~Miller,}
\author[207]{J.~Mills,}
\author[108]{O.~Mineev,}
\author[99,145]{A.~Minotti,}
\author[40]{O.~G.~Miranda,}
\author[19]{S.~Miryala,}
\author[96]{S.~Miscetti,}
\author[67]{C.~S.~Mishra,}
\author[191]{S.~R.~Mishra,}
\author[148]{A.~Mislivec,}
\author[135]{M.~Mitchell,}
\author[34]{D.~Mladenov,}
\author[172]{I.~Mocioiu,}
\author[57]{K.~Moffat,}
\author[43]{A.~Mogan,}
\author[93,16]{N.~Moggi,}
\author[83]{R.~Mohanta,}
\author[67]{T.~A.~Mohayai,}
\author[67]{N.~Mokhov,}
\author[8]{J.~Molina,}
\author[86]{L.~Molina Bueno,}
\author[93,16]{E.~Montagna,}
\author[93]{A.~Montanari,}
\author[103,67,170]{C.~Montanari,}
\author[67]{D.~Montanari,}
\author[98,185]{D.~Montanino,}
\author[40]{L.~M.~Monta{\~n}o Zetina,}
\author[209]{S.~H.~Moon,}
\author[43]{M.~Mooney,}
\author[28]{A.~F.~Moor,}
\author[5]{D.~Moreno,}
\author[104]{L.~Morescalchi,}
\author[99]{D.~Moretti,}
\author[82]{C.~Morris,}
\author[67]{C.~Mossey,}
\author[135]{M.~Mote,}
\author[210]{E.~Motuk,}
\author[65]{C.~A.~Moura,}
\author[143]{J.~Mousseau,}
\author[130]{G.~Mouster,}
\author[67]{W.~Mu,}
\author[27]{L.~Mualem,}
\author[43]{J.~Mueller,}
\author[217]{M.~Muether,}
\author[58]{F.~Muheim,}
\author[53]{A.~Muir,}
\author[22]{M.~Mulhearn,}
\author[82]{D.~Munford,}
\author[34]{L.~J.~Munteanu,}
\author[148]{H.~Muramatsu,}
\author[52]{J.~Muraz,}
\author[213]{M.~Murphy,}
\author[61]{S.~Murphy,}
\author[92]{J.~Musser,}
\author[110]{J.~Nachtman,}
\author[60]{Y.~Nagai,}
\author[136]{S.~Nagu,}
\author[221]{M.~Nalbandyan,}
\author[184]{R.~Nandakumar,}
\author[175]{D.~Naples,}
\author[116]{S.~Narita,}
\author[90]{A.~Nath,}
\author[139]{A.~Navrer-Agasson,}
\author[19]{N.~Nayak,}
\author[58]{M.~Nebot-Guinot,}
\author[116]{K.~Negishi,}
\author[218]{J.~K.~Nelson,}
\author[110]{M.~Nelson,}
\author[219]{J.~Nesbit,}
\author[67,34]{M.~Nessi,}
\author[184]{D.~Newbold,}
\author[171]{M.~Newcomer,}
\author[53]{H.~Newton,}
\author[210]{R.~Nichol,}
\author[74]{F.~Nicolas-Arnaldos,}
\author[171]{A.~Nikolica,}
\author[159]{J.~Nikolov,}
\author[67]{E.~Niner,}
\author[81]{K.~Nishimura,}
\author[67]{A.~Norman,}
\author[67]{A.~Norrick,}
\author[86]{P.~Novella,}
\author[130]{J.~A.~Nowak,}
\author[6]{M.~Oberling,}
\author[23]{J.~P.~Ochoa-Ricoux,}
\author[181]{A.~Olivier,}
\author[121]{A.~Olshevskiy,}
\author[110]{Y.~Onel,}
\author[129]{Y.~Onishchuk,}
\author[23]{J.~Ott,}
\author[22]{L.~Pagani,}
\author[59]{G.~Palacio,}
\author[67]{O.~Palamara,}
\author[34]{S.~Palestini,}
\author[67]{J.~M.~Paley,}
\author[97,72]{M.~Pallavicini,}
\author[38]{C.~Palomares,}
\author[173]{S.~Pan,}
\author[182]{W.~Panduro Vazquez,}
\author[22]{E.~Pantic,}
\author[175]{V.~Paolone,}
\author[67]{V.~Papadimitriou,}
\author[106]{R.~Papaleo,}
\author[184]{A.~Papanestis,}
\author[18]{S.~Paramesvaran,}
\author[67]{S.~Parke,}
\author[99,145]{E.~Parozzi,}
\author[13]{S.~Parsa,}
\author[19]{Z.~Parsa,}
\author[119]{S.~Parveen,}
\author[20]{M.~Parvu,}
\author[104]{D.~Pasciuto,}
\author[57,16]{S.~Pascoli,}
\author[93,16]{L.~Pasqualini,}
\author[89]{J.~Pasternak,}
\author[139]{J.~Pater,}
\author[58,210]{C.~Patrick,}
\author[93]{L.~Patrizii,}
\author[27]{R.~B.~Patterson,}
\author[131]{S.~J.~Patton,}
\author[168]{T.~Patzak,}
\author[67]{A.~Paudel,}
\author[65]{L.~Paulucci,}
\author[67]{Z.~Pavlovic,}
\author[148]{G.~Pawloski,}
\author[133]{D.~Payne,}
\author[48]{V.~Pec,}
\author[198]{S.~J.~M.~Peeters,}
\author[190]{A.~Pena Perez,}
\author[112]{E.~Pennacchio,}
\author[110]{A.~Penzo,}
\author[29]{O.~L.~G.~Peres,}
\author[57]{Y.~F.~Perez Gonzalez,}
\author[38]{L.~P{\'e}rez-Molina,}
\author[218]{C.~Pernas,}
\author[58]{J.~Perry,}
\author[56]{D.~Pershey,}
\author[99]{G.~Pessina,}
\author[190]{G.~Petrillo,}
\author[94,30]{C.~Petta,}
\author[191]{R.~Petti,}
\author[93,16]{V.~Pia,}
\author[13]{F.~Piastra,}
\author[182]{L.~Pickering,}
\author[34,102]{F.~Pietropaolo,}
\author[46,29]{V.~L.~Pimentel,}
\author[19]{G.~Pinaroli,}
\author[163]{K.~Plows,}
\author[67]{R.~Plunkett,}
\author[153,2]{T.~Pollman,}
\author[86]{F.~Pompa,}
\author[34]{X.~Pons,}
\author[111]{N.~Poonthottathil,}
\author[93,16]{F.~Poppi,}
\author[67]{S.~Pordes,}
\author[198]{J.~Porter,}
\author[19]{M.~Potekhin,}
\author[94,30]{R.~Potenza,}
\author[118]{B.~V.~K.~S.~Potukuchi,}
\author[89]{J.~Pozimski,}
\author[93,16]{M.~Pozzato,}
\author[29]{S.~Prakash,}
\author[131]{T.~Prakash,}
\author[22]{C.~Pratt,}
\author[99]{M.~Prest,}
\author[67]{F.~Psihas,}
\author[112]{D.~Pugnere,}
\author[19]{X.~Qian,}
\author[67]{J.~L.~Raaf,}
\author[19]{V.~Radeka,}
\author[18]{J.~Rademacker,}
\author[34]{R.~Radev,}
\author[222]{B.~Radics,}
\author[6]{A.~Rafique,}
\author[19]{E.~Raguzin,}
\author[215]{M.~Rai,}
\author[39]{M.~Rajaoalisoa,}
\author[67]{I.~Rakhno,}
\author[4]{A.~Rakotonandrasana,}
\author[4]{L.~Rakotondravohitra,}
\author[67]{R.~Rameika,}
\author[171]{M.~A.~Ramirez Delgado,}
\author[67]{B.~Ramson,}
\author[103,170]{A.~Rappoldi,}
\author[103,170]{G.~Raselli,}
\author[130]{P.~Ratoff,}
\author[195]{S.~Raut,}
\author[39]{H.~Razafinime,}
\author[4]{R.~F.~Razakamiandra,}
\author[148]{E.~M.~Rea,}
\author[77]{J.~S.~Real,}
\author[219,67]{B.~Rebel,}
\author[67]{R.~Rechenmacher,}
\author[139]{M.~Reggiani-Guzzo,}
\author[192]{J.~Reichenbacher,}
\author[67]{S.~D.~Reitzner,}
\author[34]{H.~Rejeb Sfar,}
\author[82]{A.~Renshaw,}
\author[19]{S.~Rescia,}
\author[34]{F.~Resnati,}
\author[200]{M.~Ribas,}
\author[100]{S.~Riboldi,}
\author[195]{C.~Riccio,}
\author[106]{G.~Riccobene,}
\author[175]{L.~C.~J.~Rice,}
\author[77]{J.~S.~Ricol,}
\author[34]{A.~Rigamonti,}
\author[61]{Y.~Rigaut,}
\author[59]{E.~V.~Rinc{\'o}n,}
\author[182]{A.~Ritchie-Yates,}
\author[134]{D.~Rivera,}
\author[67]{R.~Rivera,}
\author[77]{A.~Robert,}
\author[86]{J.~L.~Rocabado Rocha,}
\author[190]{L.~Rochester,}
\author[133]{M.~Roda,}
\author[163]{P.~Rodrigues,}
\author[34]{M.~J.~Rodriguez Alonso,}
\author[192]{J.~Rodriguez Rondon,}
\author[101]{E.~Romeo,}
\author[167]{S.~Rosauro-Alcaraz,}
\author[167]{P.~Rosier,}
\author[103,170]{M.~Rossella,}
\author[34]{M.~Rossi,}
\author[134]{M.~Ross-Lonergan,}
\author[119]{J.~Rout,}
\author[217]{P.~Roy,}
\author[61]{A.~Rubbia,}
\author[75]{C.~Rubbia,}
\author[139]{G.~Ruiz Ferreira,}
\author[131]{B.~Russell,}
\author[181]{D.~Ruterbories,}
\author[121]{A.~Rybnikov,}
\author[87]{A.~Saa-Hernandez,}
\author[210]{R.~Saakyan,}
\author[168]{S.~Sacerdoti,}
\author[91]{N.~Sahu,}
\author[100,34]{P.~Sala,}
\author[19]{N.~Samios,}
\author[121]{O.~Samoylov,}
\author[70]{M.~C.~Sanchez,}
\author[134]{V.~Sandberg,}
\author[149]{D.~A.~Sanders,}
\author[184]{D.~Sankey,}
\author[100]{D.~Santoro,}
\author[9]{N.~Saoulidou,}
\author[106]{P.~Sapienza,}
\author[39]{C.~Sarasty,}
\author[7]{I.~Sarcevic,}
\author[96]{I.~Sarra,}
\author[67]{G.~Savage,}
\author[175]{V.~Savinov,}
\author[220]{G.~Scanavini,}
\author[103]{A.~Scaramelli,}
\author[189]{A.~Scarff,}
\author[19]{A.~Scarpelli,}
\author[135]{T.~Schefke,}
\author[162,67]{H.~Schellman,}
\author[95,68]{S.~Schifano,}
\author[67]{P.~Schlabach,}
\author[36]{D.~Schmitz,}
\author[140]{A.~W.~Schneider,}
\author[56]{K.~Scholberg,}
\author[67]{A.~Schukraft,}
\author[29]{E.~Segreto,}
\author[121]{A.~Selyunin,}
\author[208]{C.~R.~Senise,}
\author[171]{J.~Sensenig,}
\author[61]{D.~Sgalaberna,}
\author[44]{M.~H.~Shaevitz,}
\author[119]{S.~Shafaq,}
\author[222]{F.~Shaker,}
\author[25]{M.~Shamma,}
\author[67]{P.~Shanahan,}
\author[207]{R.~Sharankova,}
\author[118]{H.~R.~Sharma,}
\author[19]{R.~Sharma,}
\author[178]{R.~Kumar,}
\author[198]{K.~Shaw,}
\author[67]{T.~Shaw,}
\author[112]{K.~Shchablo,}
\author[184]{C.~Shepherd-Themistocleous,}
\author[121]{A.~Sheshukov,}
\author[195]{W.~Shi,}
\author[120]{S.~Shin,}
\author[213]{I.~Shoemaker,}
\author[144]{D.~Shooltz,}
\author[195]{R.~Shrock,}
\author[131]{J.~Silber,}
\author[167]{L.~Simard,}
\author[190]{J.~Sinclair,}
\author[192]{G.~Sinev,}
\author[136]{Jaydip Singh,}
\author[136]{J.~Singh,}
\author[47]{L.~Singh,}
\author[179]{P.~Singh,}
\author[47]{V.~Singh,}
\author[166]{S.~Singh Chauhan,}
\author[34]{R.~Sipos,}
\author[93]{G.~Sirri,}
\author[192]{A.~Sitraka,}
\author[37]{K.~Siyeon,}
\author[190]{K.~Skarpaas,}
\author[92]{E.~Smith,}
\author[92]{P.~Smith,}
\author[49]{J.~Smolik,}
\author[23]{M.~Smy,}
\author[67]{E.L.~Snider,}
\author[88]{P.~Snopok,}
\author[160]{D.~Snowden-Ifft,}
\author[199]{M.~Soares Nunes,}
\author[23]{H.~Sobel,}
\author[199]{M.~Soderberg,}
\author[121]{S.~Sokolov,}
\author[107]{C.~J.~Solano Salinas,}
\author[139]{S.~S\"oldner-Rembold,}
\author[131]{S.R.~Soleti\footnote{Corresponding author.},}
\author[217]{N.~Solomey,}
\author[132]{V.~Solovov,}
\author[134]{W.~E.~Sondheim,}
\author[86]{M.~Sorel,}
\author[121]{A.~Sotnikov,}
\author[38]{J.~Soto-Oton,}
\author[39]{A.~Sousa,}
\author[35]{K.~Soustruznik,}
\author[163]{F.~Spagliardi,}
\author[99,145]{M.~Spanu,}
\author[143]{J.~Spitz,}
\author[189]{N.~J.~C.~Spooner,}
\author[199]{K.~Spurgeon,}
\author[8]{D.~Stalder,}
\author[67]{M.~Stancari,}
\author[102,165]{L.~Stanco,}
\author[22]{J.~Steenis,}
\author[18]{R.~Stein,}
\author[131]{H.~M.~Steiner,}
\author[200]{A.~F.~Steklain Lisb\^oa,}
\author[121]{A.~Stepanova,}
\author[19]{J.~Stewart,}
\author[36]{B.~Stillwell,}
\author[192]{J.~Stock,}
\author[34]{F.~Stocker,}
\author[135]{T.~Stokes,}
\author[148]{M.~Strait,}
\author[67]{T.~Strauss,}
\author[202]{L.~Strigari,}
\author[41]{A.~Stuart,}
\author[59]{J.~G.~Suarez,}
\author[15]{J.~Subash,}
\author[98]{A.~Surdo,}
\author[12]{V.~Susic,}
\author[67]{L.~Suter,}
\author[94,30]{C.~M.~Sutera,}
\author[27]{K.~Sutton,}
\author[101,150]{Y.~Suvorov,}
\author[22]{R.~Svoboda,}
\author[154]{S.~K.~Swain,}
\author[203]{B.~Szczerbinska,}
\author[58]{A.~M.~Szelc,}
\author[104]{A.~Taffara,}
\author[191]{N.~Talukdar,}
\author[5]{J.~Tamara,}
\author[190]{H. A.~Tanaka,}
\author[19]{S.~Tang,}
\author[28]{N.~Taniuchi,}
\author[205]{B.~Tapia Oregui,}
\author[89]{A.~Tapper,}
\author[67]{S.~Tariq,}
\author[19]{E.~Tarpara,}
\author[80]{N.~Tata,}
\author[84]{E.~Tatar,}
\author[92]{R.~Tayloe,}
\author[195]{A.~M.~Teklu,}
\author[131,3]{P.~Tennessen,}
\author[93]{M.~Tenti,}
\author[190]{K.~Terao,}
\author[99,145]{F.~Terranova,}
\author[97]{G.~Testera,}
\author[39]{T.~Thakore,}
\author[184]{A.~Thea,}
\author[202]{A.~Thompson,}
\author[19]{C.~Thorn,}
\author[67]{S.~C.~Timm,}
\author[19]{V.~Tishchenko,}
\author[159]{N.~Todorovi{\'c},}
\author[95,68]{L.~Tomassetti,}
\author[168]{A.~Tonazzo,}
\author[19]{D.~Torbunov,}
\author[99,145]{M.~Torti,}
\author[86]{M.~Tortola,}
\author[94,30]{F.~Tortorici,}
\author[93]{N.~Tosi,}
\author[26]{D.~Totani,}
\author[67]{M.~Toups,}
\author[133]{C.~Touramanis,}
\author[93]{R.~Travaglini,}
\author[27]{J.~Trevor,}
\author[18]{S.~Trilov,}
\author[122]{W.~H.~Trzaska,}
\author[23]{Y.~Tsai,}
\author[190]{Y.-T.~Tsai,}
\author[73]{Z.~Tsamalaidze,}
\author[190]{K.~V.~Tsang,}
\author[73]{N.~Tsverava,}
\author[117]{S.~Z.~Tu,}
\author[34]{S.~Tufanli,}
\author[131]{C.~Tull,}
\author[57]{J.~Turner,}
\author[86]{M.~Tuzi,}
\author[123]{J.~Tyler,}
\author[189]{E.~Tyley,}
\author[135]{M.~Tzanov,}
\author[34]{L.~Uboldi,}
\author[28]{M.~A.~Uchida,}
\author[92]{J.~Urheim,}
\author[190]{T.~Usher,}
\author[199]{H.~Utaegbulam,}
\author[156]{S.~Uzunyan,}
\author[124,23]{M.~R.~Vagins,}
\author[218]{P.~Vahle,}
\author[198]{S.~Valder,}
\author[63]{G.~A.~Valdiviesso,}
\author[78]{E.~Valencia,}
\author[208]{R.~Valentim,}
\author[27]{Z.~Vallari,}
\author[99]{E.~Vallazza,}
\author[86]{J.~W.~F.~Valle,}
\author[34]{S.~Vallecorsa,}
\author[171]{R.~Van Berg,}
\author[134]{R.~G.~Van de Water,}
\author[142]{D.~Vanegas Forero,}
\author[140]{D.~Vannerom,}
\author[102]{F.~Varanini,}
\author[206]{D.~Vargas Oliva,}
\author[81]{G.~Varner,}
\author[121]{S.~Vasina,}
\author[162]{N.~Vaughan,}
\author[67]{K.~Vaziri,}
\author[45]{J.~Vega,}
\author[102]{S.~Ventura,}
\author[38]{A.~Verdugo,}
\author[28]{S.~Vergani,}
\author[153]{M.~A.~Vermeulen,}
\author[67]{M.~Verzocchi,}
\author[97,72]{M.~Vicenzi,}
\author[168]{H.~Vieira de Souza,}
\author[76]{C.~Vignoli,}
\author[34]{C.~Vilela,}
\author[19]{B.~Viren,}
\author[43]{A.~Vizcaya-Hernandez,}
\author[49]{T.~Vrba,}
\author[181]{Q.~Vuong,}
\author[152]{T.~Wachala,}
\author[179]{A.~V.~Waldron,}
\author[39]{M.~Wallbank,}
\author[67]{T.~Walton,}
\author[24]{H.~Wang,}
\author[192]{J.~Wang,}
\author[131]{L.~Wang,}
\author[67]{M.H.L.S.~Wang,}
\author[67]{X.~Wang,}
\author[24]{Y.~Wang,}
\author[195]{Y.~Wang,}
\author[111]{K.~Warburton,}
\author[43]{D.~Warner,}
\author[89]{M.O.~Wascko,}
\author[210]{D.~Waters,}
\author[15]{A.~Watson,}
\author[184,198]{K.~Wawrowska,}
\author[55]{P.~Weatherly,}
\author[138,67]{A.~Weber,}
\author[13]{M.~Weber,}
\author[135]{H.~Wei,}
\author[111]{A.~Weinstein,}
\author[219]{D.~Wenman,}
\author[111]{M.~Wetstein,}
\author[220]{J.~Whilhelmi,}
\author[204]{A.~White,}
\author[220]{A.~White,}
\author[28]{L.~H.~Whitehead,}
\author[199]{D.~Whittington,}
\author[195]{M.~J.~Wilking,}
\author[210]{A.~Wilkinson,}
\author[131]{C.~Wilkinson,}
\author[204]{Z.~Williams,}
\author[184]{F.~Wilson,}
\author[43]{R.~J.~Wilson,}
\author[190]{W.~Wisniewski,}
\author[207]{J.~Wolcott,}
\author[181]{J.~Wolfs,}
\author[207]{T.~Wongjirad,}
\author[82]{A.~Wood,}
\author[131]{K.~Wood,}
\author[19]{E.~Worcester,}
\author[19]{M.~Worcester,}
\author[67]{M.~Wospakrik,}
\author[28]{K.~Wresilo,}
\author[181]{C.~Wret,}
\author[148]{S.~Wu,}
\author[67]{W.~Wu,}
\author[23]{W.~Wu,}
\author[138]{M.~Wurm,}
\author[54]{J.~Wyenberg,}
\author[23]{Y.~Xiao,}
\author[89]{I.~Xiotidis,}
\author[39]{B.~Yaeggy,}
\author[86]{N.~Yahlali,}
\author[26]{E.~Yandel,}
\author[195]{G.~Yang,}
\author[163]{K.~Yang,}
\author[67]{T.~Yang,}
\author[23]{A.~Yankelevich,}
\author[108]{N.~Yershov,}
\author[67]{K.~Yonehara,}
\author[37]{Y.~S.~Yoon,}
\author[155]{T.~Young,}
\author[19]{B.~Yu,}
\author[19]{H.~Yu,}
\author[196]{H.~Yu,}
\author[204]{J.~Yu,}
\author[88]{Y.~Yu,}
\author[58]{W.~Yuan,}
\author[222]{R.~Zaki,}
\author[48]{J.~Zalesak,}
\author[52]{L.~Zambelli,}
\author[74]{B.~Zamorano,}
\author[100]{A.~Zani,}
\author[218]{L.~Zazueta,}
\author[67]{G.~P.~Zeller,}
\author[67]{J.~Zennamo,}
\author[219]{K.~Zeug,}
\author[19]{C.~Zhang,}
\author[92]{S.~Zhang,}
\author[175]{Y.~Zhang,}
\author[19]{M.~Zhao,}
\author[19]{E.~Zhivun,}
\author[42]{E.~D.~Zimmerman,}
\author[93,16]{S.~Zucchelli,}
\author[48]{J.~Zuklin,}
\author[156]{V.~Zutshi}
\author[67]{and R.~Zwaska}

